A General Framework for Producing Interpretable Semantic Text Embeddings

Semantic text embedding is essential to many tasks in Natural Language Processing (NLP). While black-box models are capable of generating high-quality embeddings, their lack of interpretability limits their use in tasks that demand transparency. Recent approaches have improved interpretability by leveraging domain-expert-crafted or LLM-generated questions, but these methods rely heavily on expert input or well-prompt design, which restricts their generalizability and ability to generate discriminative questions across a wide range of tasks. To address these challenges, we introduce \algo{CQG-MBQA} (Contrastive Question Generation - Multi-task Binary Question Answering), a general framework for producing interpretable semantic text embeddings across diverse tasks. Our framework systematically generates highly discriminative, low cognitive load yes/no questions through the \algo{CQG} method and answers them efficiently with the \algo{MBQA} model, resulting in interpretable embeddings in a cost-effective manner. We validate the effectiveness and interpretability of \algo{CQG-MBQA} through extensive experiments and ablation studies, demonstrating that it delivers embedding quality comparable to many advanced black-box models while maintaining inherently interpretability. Additionally, \algo{CQG-MBQA} outperforms other interpretable text embedding methods across various downstream tasks.

==> tables/mteb.tex <==
\begin{table}[h]
\centering
\caption{MTEB results on different training datasets.}
\label{tab:mteb-results-different-training-datasets}
\vspace{0.5em}
\begin{tabular}{llll}
  \toprule
  \textbf{Model} & \textbf{Task} & \textbf{Dataset} & \textbf{Score} \\
  \bottomrule
\end{tabular}
\end{table}


==> tables/questions-cqg.tex <==
\begin{table}[ht]
\centering
\caption{Questions generated by CQG.}
\label{tab:questions-cqg}
\vspace{-0.5em}
\begin{tabular}{cl}
  \toprule
  \textbf{ID} & \textbf{Question} \\ \midrule
  1  & Does the article provide useful information for charging batteries? \\ 
  2  & Does the article reference specific populations at risk for deficiencies? \\
  3  & Does the article mention nudity? \\
  4  & Are there any statements of hope for normalcy returning? \\
  5  & Does the article discuss efforts to address a safety concern? \\
  6  & Is there any positive mention of public support or understanding? \\
  7  & Is there a clear relevance to sustainable practices in the article? \\
  8  & Does the article mention opportunities for discounts or special deals? \\
  9  & Is there evidence of historical impact or legacy discussed in the article? \\
  10 & Does the article mention a media platform or outlet? \\
  \bottomrule
\end{tabular}
\end{table}

==> tables/questions-qaemb.tex <==
\begin{table}[ht]
\centering
\caption{Questions generated by QAEmb.}
\label{tab:questions-qaemb}
\vspace{-0.5em}
\begin{tabular}{cl}
  \toprule
  \textbf{ID} & \textbf{Question} \\ \midrule
  1  & Does the article provide information about a specific product or its features? \\
  2  & Does the article discuss a historical event or political issue? \\
  3  & Does the article provide a historical account of an event or individual? \\
  4  & Does the article discuss a scientific or technical subject? \\
  5  & Does the article discuss a criminal case or law enforcement action? \\
  6  & Does the article discuss a specific event or occurrence? \\
  7  & Does the article discuss a specific location or geographic area? \\
  8  & Does the article explore a social or cultural event? \\
  9  & Does the article discuss a specific type of food or recipe? \\
  10 & Does the article focus on a person or a character? \\
  \bottomrule
\end{tabular}
\end{table}

